Dependency Graph Parsing as Sequence Labeling

Various linearizations have been proposed to cast syntactic dependency parsing as sequence labeling. However, these approaches do not support more complex graph-based representations, such as semantic dependencies or enhanced universal dependencies, as they cannot handle reentrancy or cycles. By extending them, we define a range of unbounded and bounded linearizations that can be used to cast graph parsing as a tagging task, enlarging the toolbox of problems that can be solved under this paradigm. Experimental results on semantic dependency and enhanced UD parsing show that with a good choice of encoding, sequence-labeling dependency graph parsers combine high efficiency with accuracies close to the state of the art, in spite of their simplicity.

==> tables/planes-iwpt.tex <==
\begin{tabular}{|c|c|cccccccccc|ccccccccccc|}
    \cline{3-23}
    \multicolumn{2}{c|}{}& \multicolumn{10}{c|}{\textbf{BiLSTM}} & \multicolumn{11}{c|}{\textbf{XLM}}\\
    \cline{2-23}
    \multicolumn{1}{c|}{} &$k$& \textbf{A} & \textbf{R} & \textbf{B\textsubscript{2}} & \textbf{B\textsubscript{3}} & \textbf{B4\textsubscript{2}} &\textbf{ B4\textsubscript{3}} & \textbf{B4\textsubscript{4}} & \textbf{B6\textsubscript{2}} & \textbf{B6\textsubscript{3}} & \textbf{B6\textsubscript{4}} & \textbf{A} & \textbf{R} & \textbf{B\textsubscript{2}} & \textbf{B\textsubscript{3}} & \textbf{B4\textsubscript{2}} &\textbf{ B4\textsubscript{3}} & \textbf{B4\textsubscript{4}} & \textbf{B6\textsubscript{2}} & \textbf{B6\textsubscript{3}} & \textbf{B6\textsubscript{4}} & \textbf{Biaf}\\
    \hline
    \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{ar}}}}
        & 1 & 54.33 & 74.80 & 77.06 & 78.37 & 77.19 & 78.62 & 78.33 & 69.55 & 78.46 & 78.99 & 83.44 & 84.99 & 90.29 & 90.26 & 90.63 & 90.30 & 90.19 & 90.31 & 90.38 & 90.85 & 92.11 \\
        & 2 & 41.44 & 70.25 & 73.35 & 73.72 & 73.00 & 74.04 & 73.55 & 66.52 & 73.85 & 74.45 & 69.43 & 80.50 & 86.59 & 86.69 & 86.49 & 86.81 & 87.18 & 86.48 & 87.27 & 87.17 & 88.66 \\
        & 3 & 39.80 & 68.87 & 72.98 & 73.75 & 72.27 & 73.84 & 73.63 & 64.24 & 74.10 & 74.29 & 66.34 & 78.65 & 85.46 & 84.82 & 85.15 & 83.93 & 86.35 & 85.12 & 85.40 & 85.06 & 87.23 \\
        & 4 & 41.85 & 60.02 & 61.99 & 63.43 & 63.14 & 64.58 & 62.43 & 58.07 & 66.60 & 64.83 & 55.25 & 69.93 & 74.93 & 74.58 & 71.46 & 73.63 & 73.86 & 70.82 & 72.01 & 74.46 & 75.44 \\
        & 5 & 24.58 & 46.70 & 39.05 & 40.45 & 42.39 & 40.45 & 38.86 & 33.12 & 38.97 & 39.77 & 28.57 & 53.33 & 60.11 & 56.35 & 55.10 & 56.38 & 51.06 & 56.70 & 50.00 & 59.46 & 55.03 \\
    % \hline 
    % \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{bg}}}}
    %     & 1 & 60.57 & 77.25 & 78.52 & 78.90 & 78.08 & 77.90 & 81.57 & 79.62 & 79.38 & 79.60 & 92.37 & 91.38 & 95.59 & 95.31 & 95.69 & 95.78 & 95.70 & 95.98 & 95.77 & 95.62 & 95.62 \\
    %     & 2 & 44.86 & 73.00 & 74.41 & 75.02 & 73.50 & 73.51 & 77.39 & 74.03 & 74.31 & 74.55 & 84.96 & 87.35 & 94.26 & 94.22 & 94.33 & 94.69 & 95.05 & 94.82 & 94.84 & 94.65 & 95.48 \\
    %     & 3 & 62.67 & 72.97 & 70.42 & 73.24 & 73.83 & 71.96 & 73.64 & 70.27 & 76.36 & 70.32 & 82.61 & 86.09 & 91.70 & 95.20 & 91.30 & 96.10 & 94.83 & 97.00 & 94.42 & 93.97 & 94.42 \\
    % \hline 
    % \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{cs}}}}
    %     & 1 & 85.61 & 87.98 & 82.40 & 82.38 & 83.14 & 83.08 & 82.86 & 82.25 & 81.97 & 81.97 & 93.94 & 94.62 & 94.75 & 94.79 & 94.75 & 94.80 & 94.70 & 94.83 & 94.80 & 94.69 & 95.24 \\
    %     & 2 & 78.53 & 83.54 & 78.26 & 78.46 & 78.49 & 78.41 & 78.35 & 78.79 & 77.96 & 78.26 & 91.86 & 92.33 & 93.55 & 93.58 & 93.65 & 93.85 & 93.86 & 94.10 & 93.91 & 93.83 & 94.83 \\
    %     & 3 & 72.19 & 78.97 & 74.08 & 73.70 & 74.27 & 73.96 & 74.13 & 74.44 & 73.69 & 73.77 & 86.11 & 87.94 & 89.50 & 90.12 & 90.14 & 91.23 & 91.05 & 90.90 & 91.36 & 91.28 & 92.88 \\
    %     & 4 & 66.85 & 72.24 & 65.88 & 67.43 & 69.34 & 71.06 & 69.19 & 69.30 & 67.36 & 67.48 & 78.33 & 80.84 & 81.15 & 82.24 & 84.38 & 85.64 & 84.89 & 84.25 & 85.68 & 84.37 & 88.60 \\
    %     & 5 & 55.70 & 71.83 & 63.91 & 64.93 & 61.48 & 60.27 & 60.24 & 67.62 & 63.91 & 62.25 & 68.00 & 75.00 & 78.72 & 79.04 & 83.00 & 84.98 & 86.23 & 82.67 & 82.61 & 85.47 & 88.42 \\
    %     & 6 & 69.84 & 80.00 & 72.13 & 66.67 & 64.52 & 62.30 & 70.77 & 67.80 & 67.80 & 58.62 & 87.88 & 77.61 & 86.15 & 87.88 & 87.88 & 92.75 & 91.18 & 91.18 & 88.24 & 94.29 & 87.88 \\
    % \hline 
    % \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{en}}}}
    %     & 1 & 61.13 & 73.84 & 74.95 & 74.80 & 75.34 & 74.60 & 74.39 & 75.46 & 75.05 & 75.62 & 89.07 & 88.25 & 91.38 & 91.54 & 91.68 & 91.34 & 91.59 & 91.22 & 91.12 & 91.24 & 91.75 \\
    %     & 2 & 53.40 & 71.95 & 73.14 & 72.93 & 73.87 & 73.04 & 73.19 & 74.06 & 73.89 & 74.52 & 85.87 & 85.84 & 90.39 & 90.24 & 90.66 & 90.82 & 90.75 & 90.49 & 90.81 & 90.95 & 91.45 \\
    %     & 3 & 46.44 & 69.51 & 70.92 & 70.51 & 70.38 & 68.94 & 70.24 & 71.88 & 71.50 & 70.70 & 81.20 & 82.75 & 87.55 & 87.32 & 87.82 & 89.02 & 89.00 & 89.55 & 88.55 & 88.75 & 91.10 \\
    %     & 4 & 68.69 & 78.00 & 68.04 & 67.35 & 77.55 & 78.43 & 74.75 & 65.98 & 70.10 & 69.39 & 91.74 & 86.24 & 83.17 & 79.61 & 81.90 & 93.46 & 92.45 & 95.33 & 94.44 & 94.44 & 88.89 \\
    % \hline 
    % \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{et}}}}
    %     & 1 & 55.32 & 69.59 & 68.41 & 65.38 & 67.30 & 66.85 & 67.53 & 67.06 & 68.42 & 68.00 & 70.04 & 87.27 & 90.15 & 90.20 & 89.96 & 90.39 & 89.98 & 90.37 & 90.28 & 90.35 & 91.99 \\
    %     & 2 & 44.47 & 64.91 & 62.57 & 60.13 & 62.76 & 62.41 & 62.46 & 63.65 & 64.22 & 64.39 & 57.13 & 82.03 & 85.51 & 85.93 & 85.86 & 86.15 & 86.08 & 86.48 & 86.21 & 85.86 & 87.90 \\
    %     & 3 & 41.88 & 59.95 & 59.00 & 56.63 & 56.88 & 57.45 & 59.41 & 57.85 & 56.70 & 59.04 & 53.30 & 79.65 & 80.67 & 84.51 & 82.80 & 83.59 & 81.23 & 82.25 & 82.49 & 82.56 & 83.92 \\
    \hline
    \parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{\textbf{fi}}}}
        & 1 & 43.93 & 63.63 & 59.96 & 61.37 & 57.95 & 59.67 & 58.89 & 60.73 & 61.23 & 61.73 & 87.58 & 87.70 & 92.13 & 92.18 & 92.24 & 92.06 & 92.02 & 92.47 & 92.05 & 92.45 & 93.44 \\
        & 2 & 35.26 & 62.07 & 59.18 & 59.74 & 56.33 & 58.16 & 57.46 & 60.14 & 58.92 & 57.96 & 81.43 & 84.27 & 90.75 & 90.57 & 91.46 & 91.27 & 91.50 & 91.85 & 91.54 & 91.76 & 93.46 \\
        & 3 & 33.30 & 59.11 & 55.69 & 57.61 & 55.09 & 56.40 & 55.46 & 60.10 & 58.14 & 57.42 & 78.65 & 81.79 & 87.91 & 88.08 & 90.41 & 90.39 & 90.10 & 90.43 & 89.88 & 90.52 & 94.47 \\
        & 4 & 25.11 & 52.39 & 46.08 & 50.15 & 45.75 & 49.79 & 48.86 & 52.54 & 55.19 & 51.00 & 68.26 & 78.24 & 82.91 & 85.57 & 83.71 & 88.17 & 91.46 & 87.27 & 90.75 & 91.78 & 94.12 \\
        & 5 & 17.86 & 42.62 & 23.53 & 26.92 & 34.48 & 32.00 & 43.64 & 43.64 & 36.36 & 45.28 & 73.33 & 61.29 & 71.43 & 72.41 & 76.67 & 74.58 & 78.69 & 75.86 & 64.41 & 77.19 & 93.75 \\
        & 6 & 17.14 & 40.00 & 31.75 & 37.50 & 31.88 & 37.14 & 28.99 & 45.07 & 42.67 & 42.67 & 52.87 & 55.81 & 61.11 & 68.42 & 60.00 & 65.85 & 62.50 & 78.48 & 66.67 & 86.05 & 96.84 \\
    \hline
    \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{fr}}}}
        & 1 & 59.68 & 74.40 & 77.41 & 77.73 & 76.75 & 76.54 & 76.92 & 77.68 & 83.78 & 77.48 & 84.12 & 83.63 & 91.67 & 91.06 & 92.78 & 93.03 & 93.16 & 93.10 & 91.98 & 93.68 & 94.02 \\
        & 2 & 39.64 & 72.15 & 73.60 & 73.29 & 74.53 & 75.09 & 74.60 & 74.71 & 78.58 & 74.86 & 69.42 & 81.18 & 88.88 & 89.06 & 90.79 & 91.07 & 90.70 & 90.83 & 90.47 & 90.27 & 93.02 \\
        & 3 & 28.59 & 70.95 & 73.13 & 72.06 & 73.61 & 73.87 & 70.88 & 74.24 & 77.22 & 75.08 & 52.69 & 78.09 & 86.96 & 85.85 & 90.79 & 89.66 & 88.64 & 89.30 & 90.32 & 89.59 & 87.90 \\
    \hline
    % \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{it}}}}
    %     & 1 & 68.53 & 82.49 & 83.46 & 83.17 & 84.48 & 84.28 & 84.32 & 84.75 & 84.10 & 83.89 & 90.82 & 91.25 & 95.36 & 95.58 & 95.80 & 95.53 & 95.76 & 95.62 & 95.72 & 95.02 & 95.76 \\
    %     & 2 & 53.72 & 76.83 & 78.63 & 78.58 & 79.64 & 78.39 & 78.70 & 79.62 & 79.34 & 80.43 & 85.88 & 85.80 & 92.47 & 92.53 & 92.93 & 93.22 & 92.71 & 92.97 & 93.08 & 92.93 & 93.82 \\
    %     & 3 & 43.41 & 73.98 & 73.68 & 71.61 & 71.12 & 71.68 & 76.97 & 74.17 & 72.18 & 74.97 & 72.39 & 81.30 & 88.89 & 88.74 & 89.23 & 89.99 & 89.27 & 92.43 & 88.60 & 92.33 & 90.04 \\
    % \hline
    % \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{lt}}}}
    %     & 1 & 35.70 & 57.71 & 58.38 & 58.00 & 55.69 & 58.11 & 57.44 & 56.41 & 57.82 & 56.56 & 73.18 & 77.51 & 87.80 & 87.54 & 87.44 & 87.83 & 87.84 & 87.40 & 88.09 & 88.51 & 90.98 \\
    %     & 2 & 26.76 & 51.74 & 49.61 & 51.92 & 48.02 & 52.06 & 50.09 & 48.94 & 50.05 & 49.61 & 64.65 & 72.73 & 84.11 & 84.50 & 85.93 & 85.76 & 84.97 & 86.18 & 85.94 & 86.10 & 89.73 \\
    %     & 3 & 20.55 & 48.77 & 46.76 & 49.07 & 45.91 & 47.17 & 45.98 & 48.52 & 50.68 & 47.44 & 47.91 & 67.41 & 76.32 & 76.78 & 79.51 & 79.41 & 78.72 & 79.11 & 78.31 & 78.18 & 86.13 \\
    %     & 4 & 25.00 & 43.04 & 40.50 & 40.28 & 41.63 & 47.31 & 39.72 & 40.09 & 44.87 & 45.98 & 57.70 & 62.00 & 72.57 & 72.44 & 73.25 & 76.82 & 74.57 & 74.78 & 74.25 & 77.22 & 78.67 \\
    %     & 6 & 11.53 & 34.42 & 33.58 & 34.53 & 28.27 & 30.24 & 34.36 & 37.80 & 37.54 & 35.33 & 33.22 & 54.89 & 65.28 & 67.82 & 65.53 & 66.67 & 65.10 & 68.61 & 63.64 & 67.96 & 76.07 \\
    % \hline 
    % \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{lv}}}}
    %     & 1 & 50.90 & 67.22 & 65.90 & 68.24 & 67.65 & 65.38 & 66.74 & 67.77 & 67.54 & 66.53 & 87.09 & 87.83 & 91.27 & 91.41 & 91.45 & 91.11 & 91.36 & 91.18 & 91.95 & 91.76 & 93.48 \\
    %     & 2 & 36.07 & 60.88 & 60.68 & 61.92 & 62.14 & 58.98 & 59.66 & 61.41 & 60.49 & 60.55 & 80.31 & 83.93 & 90.17 & 90.00 & 91.13 & 90.80 & 91.25 & 90.74 & 90.99 & 91.24 & 93.08 \\
    %     & 3 & 30.68 & 56.90 & 55.98 & 57.82 & 58.00 & 56.10 & 56.08 & 57.35 & 57.23 & 56.90 & 71.47 & 78.57 & 86.54 & 86.32 & 87.50 & 88.48 & 88.46 & 87.30 & 88.51 & 88.30 & 91.86 \\
    %     & 4 & 26.71 & 52.16 & 54.39 & 56.26 & 57.00 & 54.61 & 56.86 & 56.63 & 54.09 & 52.06 & 61.77 & 72.46 & 77.57 & 75.91 & 78.05 & 81.45 & 84.76 & 80.85 & 82.07 & 82.16 & 91.57 \\
    %     & 5 & 8.21 & 43.48 & 43.58 & 43.24 & 46.10 & 40.29 & 41.88 & 44.19 & 45.98 & 44.11 & 51.05 & 59.72 & 72.06 & 68.31 & 73.68 & 74.13 & 78.72 & 72.66 & 68.61 & 70.04 & 83.22 \\
    % \hline
    % \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{nl}}}}
    %     & 1 & 60.57 & 76.04 & 73.97 & 74.65 & 76.40 & 75.45 & 76.25 & 76.75 & 76.25 & 77.08 & 92.52 & 91.37 & 94.09 & 94.08 & 94.28 & 94.04 & 94.46 & 94.38 & 93.95 & 94.13 & 93.83 \\
    %     & 2 & 46.77 & 68.61 & 66.72 & 67.52 & 68.87 & 67.33 & 67.96 & 69.53 & 70.16 & 70.18 & 87.64 & 86.91 & 92.03 & 91.91 & 92.64 & 92.60 & 92.34 & 92.77 & 93.06 & 93.66 & 93.04 \\
    %     & 3 & 41.59 & 65.22 & 63.29 & 63.68 & 64.24 & 63.50 & 66.80 & 65.02 & 64.41 & 64.81 & 83.33 & 84.85 & 89.50 & 88.60 & 91.50 & 91.78 & 91.48 & 91.73 & 92.53 & 92.04 & 93.03 \\
    % \hline
    % \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{pl}}}}
    %     & 1 & 68.84 & 80.56 & 78.60 & 78.67 & 77.80 & 77.33 & 76.80 & 79.82 & 78.28 & 79.22 & 94.65 & 94.09 & 94.97 & 95.07 & 95.17 & 95.13 & 95.29 & 95.21 & 95.13 & 95.14 & 96.38 \\
    %     & 2 & 49.55 & 70.85 & 70.07 & 69.93 & 69.29 & 69.34 & 67.97 & 71.10 & 70.11 & 71.06 & 90.65 & 89.27 & 92.52 & 92.84 & 93.44 & 93.46 & 93.44 & 93.25 & 93.33 & 93.33 & 94.85 \\
    %     & 3 & 39.78 & 64.29 & 63.61 & 64.45 & 63.71 & 62.87 & 61.20 & 65.30 & 63.70 & 65.65 & 83.93 & 84.59 & 88.37 & 89.71 & 90.24 & 91.29 & 91.79 & 90.69 & 91.02 & 91.64 & 93.73 \\
    %     & 4 & 32.24 & 61.70 & 59.24 & 61.17 & 59.83 & 60.58 & 59.70 & 60.36 & 59.48 & 61.75 & 76.67 & 75.60 & 83.37 & 84.46 & 87.01 & 87.05 & 86.94 & 86.05 & 88.19 & 87.97 & 92.18 \\
    %     & 5 & 33.12 & 64.67 & 52.90 & 55.00 & 55.13 & 57.32 & 52.23 & 64.63 & 54.43 & 63.03 & 66.67 & 64.71 & 64.67 & 67.47 & 66.67 & 65.06 & 61.82 & 63.47 & 62.28 & 66.27 & 64.74 \\
    % \hline
    % \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{ru}}}}
    %     & 1 & 69.11 & 80.53 & 77.48 & 77.36 & 77.93 & 76.48 & 77.50 & 77.91 & 77.71 & 82.27 & 94.72 & 94.83 & 95.57 & 95.56 & 95.55 & 95.50 & 95.55 & 95.59 & 95.66 & 95.71 & 96.41 \\
    %     & 2 & 59.18 & 74.80 & 73.38 & 72.24 & 73.53 & 71.77 & 72.40 & 74.16 & 74.14 & 78.09 & 92.32 & 91.96 & 94.22 & 94.25 & 94.11 & 94.32 & 94.26 & 94.57 & 94.62 & 94.65 & 95.43 \\
    %     & 3 & 53.16 & 72.48 & 71.05 & 70.09 & 71.86 & 69.45 & 70.19 & 70.38 & 71.15 & 74.96 & 90.79 & 89.22 & 92.37 & 92.66 & 93.23 & 93.48 & 93.60 & 92.91 & 93.87 & 93.04 & 94.74 \\
    %     & 4 & 45.80 & 59.26 & 57.60 & 61.90 & 60.00 & 56.49 & 58.02 & 61.42 & 56.92 & 62.02 & 87.41 & 88.89 & 90.37 & 91.97 & 94.12 & 94.89 & 87.41 & 91.18 & 89.71 & 94.12 & 94.89 \\
    % \hline
    \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{sk}}}}
        & 1 & 46.49 & 65.75 & 65.67 & 63.38 & 67.42 & 65.21 & 66.27 & 67.47 & 66.15 & 65.97 & 89.41 & 90.21 & 94.51 & 94.73 & 94.38 & 94.93 & 94.71 & 94.61 & 94.83 & 94.51 & 94.43 \\
        & 2 & 35.61 & 62.97 & 62.60 & 60.09 & 64.95 & 60.81 & 62.38 & 65.87 & 65.69 & 64.86 & 78.73 & 84.24 & 92.87 & 93.06 & 93.63 & 93.83 & 93.55 & 94.00 & 94.20 & 93.69 & 94.27 \\
        & 3 & 32.74 & 58.30 & 56.95 & 53.06 & 60.78 & 58.76 & 58.97 & 61.33 & 62.90 & 61.56 & 74.96 & 78.64 & 87.66 & 88.85 & 90.84 & 90.09 & 89.94 & 90.37 & 90.46 & 91.49 & 93.16 \\
        & 4 & 38.96 & 64.20 & 72.97 & 74.67 & 61.11 & 65.71 & 61.33 & 72.00 & 64.20 & 65.82 & 76.54 & 82.35 & 80.00 & 94.12 & 92.86 & 85.00 & 91.57 & 89.16 & 91.57 & 83.54 & 92.86 \\
        & 5 & 22.45 & 58.82 & 52.75 & 43.18 & 47.92 & 43.18 & 47.42 & 52.08 & 40.40 & 47.31 & 29.13 & 71.15 & 74.75 & 76.77 & 75.51 & 76.92 & 74.51 & 84.00 & 80.81 & 78.00 & 77.78 \\
    \hline
    % \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{sv}}}}
    %     & 1 & 41.83 & 66.70 & 71.17 & 70.94 & 67.47 & 71.46 & 78.48 & 69.91 & 69.97 & 69.18 & 81.42 & 83.85 & 90.00 & 90.21 & 91.36 & 91.61 & 91.18 & 91.56 & 91.29 & 91.12 & 92.30 \\
    %     & 2 & 33.92 & 63.70 & 67.95 & 67.58 & 63.30 & 67.96 & 75.62 & 66.14 & 66.42 & 65.25 & 72.71 & 78.95 & 86.56 & 86.83 & 88.85 & 89.00 & 88.54 & 88.77 & 89.05 & 88.78 & 90.01 \\
    %     & 3 & 28.36 & 65.41 & 66.69 & 67.90 & 62.97 & 68.66 & 75.14 & 65.84 & 67.64 & 65.20 & 60.09 & 76.23 & 84.80 & 83.60 & 83.66 & 84.81 & 84.25 & 85.54 & 85.19 & 84.39 & 87.44 \\
    %     & 4 & 16.58 & 55.38 & 57.92 & 54.75 & 55.56 & 59.79 & 56.38 & 52.41 & 50.79 & 58.38 & 45.23 & 66.99 & 75.90 & 75.51 & 81.59 & 78.61 & 80.79 & 77.16 & 81.41 & 82.18 & 81.16 \\
    % \hline
    \parbox[t]{2mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\textbf{ta}}}}
        & 1 & 34.90 & 61.82 & 64.83 & 64.83 & 67.45 & 67.89 & 67.89 & 71.76 & 71.76 & 71.76 & 36.84 & 66.37 & 74.57 & 74.57 & 76.54 & 77.23 & 77.23 & 77.65 & 77.65 & 77.65 & 78.49 \\
        & 2 & 17.08 & 53.20 & 49.54 & 49.54 & 53.79 & 52.52 & 52.52 & 52.84 & 52.84 & 52.84 & 19.83 & 55.21 & 68.06 & 68.06 & 71.60 & 69.04 & 69.04 & 67.56 & 67.56 & 67.56 & 63.43 \\
    \hline
    % \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\textbf{uk}}}}
    %     & 1 & 40.34 & 63.31 & 61.48 & 59.93 & 64.66 & 63.73 & 62.52 & 63.71 & 62.31 & 62.83 & 81.79 & 85.92 & 93.37 & 93.12 & 93.35 & 93.49 & 93.06 & 93.29 & 93.45 & 93.42 & 95.21 \\
    %     & 2 & 26.90 & 60.02 & 58.00 & 56.02 & 59.69 & 58.66 & 57.84 & 59.76 & 60.68 & 58.31 & 65.13 & 80.39 & 89.48 & 89.58 & 90.39 & 90.52 & 90.54 & 91.06 & 90.97 & 90.65 & 92.83 \\
    %     & 3 & 20.96 & 55.89 & 54.67 & 53.70 & 56.95 & 56.80 & 55.37 & 55.18 & 55.74 & 55.71 & 55.49 & 75.79 & 83.53 & 84.62 & 87.00 & 87.40 & 85.49 & 86.45 & 86.86 & 86.04 & 89.88 \\
    %     & 4 & 19.67 & 58.39 & 54.87 & 55.74 & 61.19 & 56.45 & 58.06 & 60.00 & 64.41 & 59.68 & 63.31 & 69.44 & 81.16 & 78.83 & 80.00 & 81.43 & 81.75 & 78.57 & 80.00 & 79.17 & 83.78 \\
    %     & 5 & 11.27 & 40.00 & 29.03 & 30.99 & 32.88 & 41.98 & 42.67 & 25.32 & 35.44 & 30.95 & 64.20 & 60.98 & 77.92 & 73.42 & 71.05 & 82.93 & 77.11 & 86.75 & 71.05 & 78.95 & 86.75 \\
    % \hline
\end{tabular}
